Minimal spin deflection of Kerr-Newman and Supersymmetric black hole

Recent studies have shown that minimal couplings for massive spinning particles, which in the classical limit reproduce the leading PM Kerr black hole dynamics, leads to an Eikonal S-matrix exhibiting spin-entanglement suppression. In this paper we trace this phenomenon to the suppression of spin-flipping components in the S-matrix, known to be the hallmark of minimal coupling in the ultra-relativistic limit. We further generalize the consideration to charged and $\mathcal{N}=4$ black holes, demonstrating that in both cases maximal suppression occurs at the extremal limit.

==> 3pt_diagram_scalar.tex <==

\tikzset{
  photon/.style={decorate, decoration={snake}, draw=black},
  fermion/.style={draw=black, postaction={decorate},decoration={markings,mark=at position .55 with {\arrow{>}}}},
}





\begin{figure}[H]
\label{fig: 3-pt vertex}
\centering
\begin{tikzpicture}[node distance=0.5cm and 0.5cm]
\coordinate[] (v1);
\coordinate[right=of v1] (v2);
\coordinate[right=of v2] (v3);
\coordinate[right= of v3] (v4);
\coordinate[above left = 1.5cm and 1.5cm of v1,label=left :$\bold{1}^{\{I_1\cdots I_{2s}\}}$ ] (e1);
\coordinate[below left = 1.5cm and 1.5cm of v1,label=left :$\bold{2}^{\{J_1\cdots J_{2s}\}}$ ] (e2);
\draw[fermion] (e1) -- (v1) node[midway, sloped, above=0.1cm,font=\footnotesize] {\tiny$p_1,m,(Z_{12},Z_{34})$};
\draw[fermion] (e2) -- (v1) node[midway, sloped, below=0.1cm,font=\footnotesize] {\tiny$p_2,m,(-Z_{12},-Z_{34})$};
\draw[photon] (v1) -- (v4) node[midway,below=0.1cm] {$\longleftarrow$} node[right] {$h$  } node[midway, above=0.1cm]{$P$};
\end{tikzpicture}
\caption{A 3-pt super amplitude of two massive spin-s multiplets with equal mass $m$ and a massless particle with helicity $h$ multiplet.}
\end{figure}




==> FeynmanDiagram.tex <==





\begin{figure}[H]
\centering
\begin{tikzpicture}[node distance=1cm and 1cm]
\coordinate[] (v1);
\coordinate[right=of v1] (v2);
\coordinate[right=of v2] (v3);
\coordinate[right= of v3] (v4);
\coordinate[above right= 2cm and 2cm of v4,label=right:$\bm{2}^\prime_{\text{spin-0}}$] (f1);
\coordinate[below right= 2cm and 2cm of v4,label=right:$\bm{2}_{\text{spin-0}}$] (f2);
\coordinate[above left = 2cm and 2cm of v1,label=left :$\bm{1}^{\prime\{I^\prime_1\cdots I^\prime_{4}\}}_{\text{spin-2}}$] (e1);
\coordinate[below left = 2cm and 2cm of v1,label=left :$\bm{1}^{\{I_1\cdots I_{4}\}}_{\text{spin-2}}$] (e2);
\draw[fermion] (v1) -- (e1) node[midway, sloped, above=0.1cm,font=\footnotesize] {$p_3, m_1, Z_1$};
\draw[fermion] (e2) -- (v1) node[midway, sloped, below=0.1cm,font=\footnotesize] {$p_1, m_1, Z_1$};
\draw[photon] (v1) -- (v4) node[midway,below=0.1cm] {$\longrightarrow$} node[midway, above=0.1cm]{$q$};
\draw[fermion] (v4) -- (f1) node[midway, sloped, above=0.1cm,font=\footnotesize] {$p_4, m_2, Z_2$};
\draw[fermion] (f2) -- (v4) node[midway, sloped, below=0.1cm,font=\footnotesize] {$p_2, m_2, Z_2$};
\end{tikzpicture}
\caption{The exchange of a supermultiplet between spin-2 and a scalar particle with transfer momentum $q$.}
\label{4ptgraph}
\end{figure}




